History repeats Itself: A Baseline for Temporal Knowledge Graph Forecasting

Temporal Knowledge Graph (TKG) Forecasting aims at predicting links in Knowledge Graphs for future timesteps based on a history of Knowledge Graphs. To this day, standardized evaluation protocols and rigorous comparison across TKG models are available, but the importance of simple baselines is often neglected in the evaluation, which prevents researchers from discerning actual and fictitious progress. We propose to close this gap by designing an intuitive baseline for TKG Forecasting based on predicting recurring facts. Compared to most TKG models, it requires little hyperparameter tuning and no iterative training. Further, it can help to identify failure modes in existing approaches. The empirical findings are quite unexpected: compared to 11 methods on five datasets, our baseline ranks first or third in three of them, painting a radically different picture of the predictive quality of the state of the art.

==> chapters/sup_tables/table_alpha.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table*} 
%\scriptsize
\centering
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r|r}
\toprule
$\alpha$  &0         & 1.00E-05  & 0.0001    & 0.001     & 0.01      & 0.1       & 0.5       & 0.9       & 0.99      & 0.999     & 0.9999    & 0.99999   & 1        \\ % & -1     \\   %& -2   \\
MRR  & 14.4      & 14.6     & 14.6     & 14.6    & 14.8     & 17.5    & 27.0     & 34.7    & 35.9     & 36.6    & 37.1     & 37.2      & 37.2   \\ %   & 36.64   \\  %& 37.19 \\ % 22.12.
% updated 22.12.
\bottomrule
  \end{tabular}
  \caption{Test MRR for the \rb ($\psi_{\Delta_{\lambda=0.04}}\xi$) for different values of $\alpha$. Example for dataset ICEWS14.}
\label{table:paramvaluesalpha}
\end{table*}

==> chapters/sup_tables/table_lambda.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table*} 
%\scriptsize
\centering
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\toprule
%\multicolumn{14}{l}{ $\psi_\Delta$ }    \\
%\midrule 
% \begin{tabular}{lllllllllllllllllllll}
$\lambda$  & 0         & 0.0001    & 0.0005    & 0.001     & 0.005     & 0.01      & 0.02      & 0.04      & 0.06      & 0.08      & 0.1       & 0.5       & 0.9       & 1.0001     \\
 MRR & 34.4     & 35.3    & 35.3     & 35.3     & 35.6     & 35.7     & 35.9     & 36.0     & 36.0     & 35.9     & 35.5     & 30.3     & 27.9     & 27.5     \\ %updated on 22.12. 
\bottomrule
  \end{tabular}
  \caption{Test MRR for the \srb ($\psi_\Delta$) for different values of $\lambda$. Example for dataset ICEWS14.}
\label{table:paramvalueslambda}
\end{table*}

==> chapters/sup_tables/table_multistep.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table*} 
%\scriptsize
\centering
\begin{tabular}{l|rr|rr|rr|rr|rr}
\toprule
& \multicolumn{2}{c|}{GDELT} & \multicolumn{2}{c|}{YAGO} & \multicolumn{2}{c|}{WIKI} & \multicolumn{2}{c|}{ICEWS14} & \multicolumn{2}{c}{ICEWS18} \\
\midrule
		                  & MRR  & H@10 & MRR  & H@10 & MRR  & H@10 & MRR & H@10 & MRR & H@10  \\
\midrule
RE-GCN                                                                     & 19.6          & 33.6          & 75.4          & 81.7          & 62.7          & 67.9          & \textbf{37.8} & \textbf{57.5} & \textbf{29.0} & \textbf{47.5} \\
RE-Net                                                                     & \textbf{19.7} & \textbf{33.9} & 58.2          & 66.3          & 49.5          & 53.0          & 37.0          & 54.9          & 27.9          & 46.2          \\
CyGNet                                                                     & 19.1          & 33.1          & 69.0          & 83.4          & 58.3          & 67.6          & 36.1          & 54.5          & 26.0          & 44.4          \\
TLogic                                                                     & 17.7          & 30.3          & 66.9          & 71.6          & 64.0          & 68.2          & 35.5          & 53.1          & 24.0          & 41.2          \\
\midrule
$\xi$             & 14.1          & 23.4          & 5.1           & 10.5          & 14.0          & 24.7          & 14.1          & 27.8          & 11.6          & 21.8          \\
$\psi_\Delta$           & 18.1          & 30.4          & 81.4          & 84.2          & 63.7          & 68.2          & 30.1          & 40.8          & 23.4          & 35.8          \\
$\psi_\Delta\xi$   & 19.2          & 32.5          & \textbf{81.7} & \textbf{84.6} & \textbf{64.3} & \textbf{69.0} & 31.7          & 45.4          & 24.6          & 38.6     \\    

\bottomrule
  \end{tabular}
  \caption{Experimental results for multi-step prediction.
}
\label{table:results_multistep}
\end{table*}


==> chapters/sup_tables/table_psi_lambda_alldatasets.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table*} 
%\scriptsize
\centering
\begin{tabular}{l|rr|rr|rr|rr|rr}
\toprule
& \multicolumn{2}{c|}{GDELT} & \multicolumn{2}{c|}{YAGO} & \multicolumn{2}{c|}{WIKI} & \multicolumn{2}{c|}{ICEWS14} & \multicolumn{2}{c}{ICEWS18} \\
\midrule
		                                      & MRR  & H@10 & MRR  & H@10 & MRR  & H@10 & MRR & H@10 & MRR & H@10  \\
\midrule
$\psi_{\Delta_{\lambda=0}} \Leftrightarrow \psi_{1}$         & 20.8 & 35.3 & 81.6 & 90.9 & 68.1 & 83.5 & 34.4 & 47.2 & 26.2 & 40.3 \\ %updated 22.12. baselinepsi_singlestep_0.0_1.0_1.0
$\psi_{\Delta_{\lambda=0.1}}$                                & 19.5 & 31.3 & 85.7 & 92.3 & 73.7 & 85.6 & 35.5 & 47.8 & 26.8 & 40.4 \\ %updated 22.12.  baselinepsi_singlestep_0.1_1.0_1.0
$\psi_{\Delta_{\lambda=1.0001}} \Leftrightarrow  \phi_{\Delta}$   & 12.1 & 18.3 & 90.7 & 92.8 & 81.6 & 87.0 & 27.5 & 33.8 & 21.0 & 29.9 \\  %updated 22.12. baselinepsi_singlestep_1.0001_1.0_1.0
$\psi_{\Delta_{\lambda_r (\texttt{per rel})}}$          & 23.7 & 38.3 & 90.7 & 92.8 & 81.6 & 87.0 & 36.3 & 48.4 & 27.8 & 41.4 \\ % update 22.12. baselinepsi_singlestep_-1_-1_0.0001 and baselinepsi_singlestep_-1_-1_1.0 (same configuration)
\bottomrule
  \end{tabular}
  \caption{Experimental results for single-step prediction on the \srb $\psi$ for different time decay settings, i.e. for different values of~$\lambda$.}
\label{table:resultsperlambda}
\end{table*}

==> chapters/sup_tables/table_selected_lambdas.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table*} 

%\scriptsize
\centering
\begin{tabular}{l|r|r|r|r|r}
\toprule
            & {GDELT} & {YAGO}      & {WIKI}    & {ICEWS14} & {ICEWS18} \\
\midrule
$\lambda$   & 0.01   & 1.0001      & 1.0001    & 0.02      & 0.02    \\
$\alpha$    & 0.99    & 0.99         & 0.99999   & 0.999    & 0.99     \\ % updated 2.1.2024
% $\lambda$   & 0.005   & 1.0001      & 1.0001    & 0.02      & 0.01    \\
% $\alpha$    & 0.99    & 0.5         & 0.99999   & 0.9999    & 0.99     \\
\bottomrule
  \end{tabular}
  \caption{Values for parameters $\lambda$ and $\alpha$ that have been selected per dataset when stipulating values for $\lambda$ and $\alpha$ across all relations.}
\label{table:paramvalues}
\end{table*}

